Unbiased Scene Graph Generation in Videos

The task of dynamic scene graph generation (SGG) from videos is complicated and challenging due to the inherent dynamics of a scene, temporal fluctuation of model predictions, and the long-tailed distribution of the visual relationships in addition to the already existing challenges in image-based SGG. Existing methods for dynamic SGG have primarily focused on capturing spatio-temporal context using complex architectures without addressing the challenges mentioned above, especially the long-tailed distribution of relationships. This often leads to the generation of biased scene graphs. To address these challenges, we introduce a new framework called TEMPURA: TEmporal consistency and Memory Prototype guided UnceRtainty Attenuation for unbiased dynamic SGG. TEMPURA employs object-level temporal consistencies via transformer-based sequence modeling, learns to synthesize unbiased relationship representations using memory-guided training, and attenuates the predictive uncertainty of visual relations using a Gaussian Mixture Model (GMM). Extensive experiments demonstrate that our method achieves significant (up to 10% in some cases) performance gain over existing methods highlighting its superiority in generating more unbiased scene graphs.

==> mR_sota_sgdet.tex <==

\begin{table}[]
\centering
\caption{Comparative results for SGDET task, on AG \cite{Action_genome_Ji_2020_CVPR}, in terms of mRecall@K. 
$\dagger$ denotes our reproduced results for the same evaluation setup.}
\setlength{\tabcolsep}{12pt}
\resizebox{1\linewidth}{!}
{%
\begin{tabular}{ccccccc}
% \hline
\toprule
  \multirow{2}{*}{Method} & \multicolumn{3}{c}{With Constraint} & \multicolumn{3}{c}{No Constraints}\\
  \cmidrule(lr){2-4} \cmidrule(lr){5-7}   
  &mR@10 &mR@20 &mR@50 &mR@10 &mR@20 &mR@50 
\\
\midrule
\midrule
  RelDN~\cite{zhang2019vrd}$\dagger$ & 3.3 & 3.3 & 3.3 & 7.5 & 18.8 & 33.7 \\
  HCRD supervised\cite{simple_baseline_bmvc} & - & 8.3 & 9.1& - &  - & - \\
  TRACE\cite{teng2021target}& 8.2 & 8.2 & 8.2  & 22.8 &31.3 & 41.8\\
  ISGG \cite{ISG_arxiv22} & - & 19.7 & 22.9 & - & - & - \\
  STTran\cite{STTran_2021}&  16.6 & 20.8 & 22.2 & 20.9 & 29.7 & 39.2  \\
  STTran-TPI \cite{TPI_MM_22}& 15.6 & 20.2 & 21.8 & - & - & - \\
  TEMPURA& \textbf{ 18.5} &\textbf{ 22.6} & \textbf{23.7} &  \textbf{24.7} & \textbf{33.9} & \textbf{43.7}  \\
\bottomrule
\end{tabular}
\label{tab:mR_sota_sgdet}}
\vspace{-5mm}
\end{table}

==> predictive_uncertainty.tex <==
\begin{figure}[h]
\centering
\begin{subfigure}[b]{0.4\linewidth}
  \centering
  \includegraphics[width=1\textwidth]{figs/jpegs/al_vs_epoch.jpg}  
  \caption{}
\end{subfigure}
\begin{subfigure}[b]{0.4\linewidth}
  \centering
  \includegraphics[width=1\textwidth]{figs/jpegs/ep_vs_epoch.jpg}
  \caption{}
\end{subfigure}
\caption{Total predictive uncertainty of TEMPURA with each training epoch, for the SGDET task. Both uncertainties are computed by averaging over all samples over all predicate classes. 
% From the overall graph, it can be ascertained 
We observe that the model progressively learns to attenuate the effect of high uncertainty caused due to noisy SGG data.  }
\vspace{-1em}
\label{fig:predictive_uncertainty}
\end{figure}  
